On Mirzakhani's twist torus conjecture

We address a conjecture of Mirzakhani about the statistical behavior of certain expanding families of ``twist tori'' in the moduli space of hyperbolic surfaces, showing that they equidistribute to a certain Lebesgue-class measure along almost all sequences. We also identify a number of other expanding families of twist tori whose limiting distributions are mutually singular to Lebesgue.

==> packages.tex <==

\usepackage{amssymb, amsfonts, amsmath, amsthm,bm, amscd}
\usepackage[dvipsnames]{xcolor}
\usepackage{mathrsfs}
%\usepackage{hyperref}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage[margin=1.00 in]{geometry}
\usepackage{enumitem, multicol}
\usepackage{tikz}
\usetikzlibrary{cd}
\usepackage{nicefrac, bigints}
\usepackage{array}
\usepackage{stmaryrd}
\usepackage{mathtools} 
\usepackage{extarrows} 
\usepackage{amsbsy}
\usepackage{bbm}

\usepackage[colorlinks,citecolor=cyan,linkcolor=teal]{hyperref}


%\usepackage{biblatex}
%\addbibresource{references/references_SHSH.bib}
%\bibliographystyle{amsalpha.bst}
%\bibliography{references_SHSH}{}

\renewcommand{\thepart}{\Roman{part}} 
\newcommand{\para}[1]{\medskip\noindent\textbf{#1.}}

\theoremstyle{definition}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{maintheorem}{Theorem}
\renewcommand{\themaintheorem}{\Alph{maintheorem}}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{sublemma}[theorem]{Sublemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{question}[theorem]{Question}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{example}[theorem]{Example}
\newtheorem*{notation}{Notation}

\makeatletter
\DeclareRobustCommand{\cev}[1]{%
  {\mathpalette\do@cev{#1}}%
}
\newcommand{\do@cev}[2]{%
  \vbox{\offinterlineskip
    \sbox\z@{$\m@th#1 x$}%
    \ialign{##\cr
      \hidewidth\reflectbox{$\m@th#1\vec{}\mkern4mu$}\hidewidth\cr
      \noalign{\kern-\ht\z@}
      $\m@th#1#2$\cr
    }%
  }%
}
\makeatother

\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\ith}{^\text{th}}
\newcommand{\inverse}{^{-1}}

\newcommand{\cN}{\mathcal{N}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cP}{\mathcal{P}}

\DeclareMathOperator{\Mod}{Mod}
\newcommand{\PMF}{\mathcal{PMF}}
\newcommand{\MF}{\mathcal{MF}}
\newcommand{\PML}{\mathcal{PML}}
\newcommand{\ML}{\mathcal{ML}}
\newcommand{\MLp}{\mathcal{ML}_\text{poly}}
\newcommand{\GL}{\mathsf{GL}}
\DeclareMathOperator{\GLcr}{\mathcal{GL}^{cr}}
\DeclareMathOperator{\GLcrmax}{\mathcal{GL}^{cr}_{max}}
\newcommand{\SL}{\mathsf{SL}}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\core}{core}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\Lip}{Lip}
\DeclareMathOperator{\vol}{vol}

\newcommand{\sB}{\mathscr{B}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\A}{\mathsf{A}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\HT}{\mathcal{HT}}
\newcommand{\HM}{\mathcal{HM}}
\newcommand{\PT}{\mathcal{PT}}
\newcommand{\PM}{\mathcal{PM}}
\newcommand{\PoT}{\mathcal{P}^1\mathcal{T}}
\newcommand{\PoM}{\mathcal{P}^1\mathcal{M}}
\newcommand{\QT}{\mathcal{QT}}
\newcommand{\QM}{\mathcal{QM}}
\newcommand{\QoT}{\mathcal{Q}^1\mathcal{T}}
\newcommand{\QoM}{\mathcal{Q}^1\mathcal{M}}
\newcommand{\sing}{\underline{\kappa}}
\newcommand{\RG}{\mathfrak{R}}

\newcommand{\fcH}{\underline{\mathcal H}}
\newcommand{\epN}[1]{\mathcal{N}_\epsilon(#1)}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\SH}{\mathcal{SH}}
\DeclareMathOperator{\Sp}{\mathsf{Sp}}
\DeclareMathOperator{\val}{val}
\DeclareMathOperator{\Isom}{Isom}
\DeclareMathOperator{\PSL}{\mathsf{PSL}}
\DeclareMathOperator{\str}{stretch}
\DeclareMathOperator{\inj}{inj}
\DeclareMathOperator{\Area}{Area}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\cen}{center}

\newcommand{\tlambda}{\widetilde{\lambda}}
\newcommand{\tX}{\widetilde{X}}
\newcommand{\partiall}{\partial_\lambda}
\newcommand{\tQ}{\widetilde{Q}}
\newcommand{\tS}{\widetilde{S}}
\newcommand{\tSp}{\widetilde{\Sp}}
\newcommand{\vtSp}{\widetilde{\Sp}{}^{(0)}}
\newcommand{\tlambdaa}{\widetilde{\lambda_{\arc}}}
\newcommand{\lambdaa}{\lambda_{\arc}}
\newcommand{\taua}{\tau_{\arc}}
\newcommand{\ttau}{\widetilde{\tau}}
\newcommand{\ttaua}{\widetilde{\tau_{\arc}}}
\newcommand{\sigl}{\sigma_\lambda}
\newcommand{\ac}{\mathfrak{s}}
\newcommand{\acarc}{\mathfrak{a}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\Defl}{\mathcal{D}_\lambda}
\newcommand{\frakML}{\mathfrak{ML}}
\DeclareMathOperator{\Ol}{\mathcal{O}_\lambda}
\DeclareMathOperator{\Il}{I_\lambda}
\DeclareMathOperator{\lk}{lk}
\DeclareMathOperator{\Per}{Per}

\newcommand{\ribs}{\mathsf{Y}}
\newcommand{\rib}{y}

\newcommand{\arc}{\underline{\alpha}}
\newcommand{\arcwt}{\underline{A}}
\newcommand{\arcb}{\underline{\beta}}
\newcommand{\arcwtb}{\underline{B}}
\newcommand{\arcc}{\underline{\gamma}}

\DeclareMathOperator{\supp}{supp}
\newcommand{\Arc}{\mathscr{A}}
\newcommand{\Arcfill}{\mathscr{A}_\text{fill}}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Stab}{Stab}
\newcommand{\crowns}{\{\underline{c}\}}
\newcommand{\Crown}{\mathcal{C}}
\newcommand{\Fol}{\mathcal W}
\newcommand{\cutsurf}{\Sigma}
\newcommand{\Base}{\mathscr{B}(S \setminus \lambda)}
\DeclareMathOperator{\ThH}{\omega_{\calH}}
\DeclareMathOperator{\ThSH}{\omega_{\SH}}
\DeclareMathOperator{\res}{res}
\DeclareMathOperator{\trem}{trem}
\DeclareMathOperator{\Eq}{Eq}
\DeclareMathOperator{\Str}{Str}
\DeclareMathOperator{\Sch}{Sch}
\DeclareMathOperator{\ext}{ext}

\DeclareMathOperator{\WP}{WP}
\DeclareMathOperator{\Th}{Th}
\DeclareMathOperator{\MV}{MV}
\DeclareMathOperator{\reg}{reg}
\DeclareMathOperator{\snug}{snug}
\newcommand{\kTh}{\mu^{\Th}_{\cQ}}

\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}

\newcommand{\TT}{\mathbb{T}}
\newcommand{\OT}{\mathcal{O}\mathbb{T}}
\newcommand{\OTg}{\mathcal{O}\mathbb{T}_{\gamma}}
\newcommand{\LL}{\mathbf{L}}
\newcommand{\scrR}{\mathscr{R}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\abc}{m}
\newcommand{\cL}{\mathcal L}
\DeclareMathOperator{\hol}{hol}
\DeclareMathOperator{\ImAnn}{ImAnn}


%The following gives us a way to put notes in!
\newcommand{\aaron}[1]{{\color{blue} \sf  A: [#1]}}
\newcommand{\james}[1]{{\color{red} \sf  J: [#1]}}
\newcommand{\revise}[1]{{\color{purple} \sf  [#1]}}
\newcommand{\cn}{{\color{green} \sf [Citation Needed]}}
\colorlet{lgray}{gray!40}
\newcommand{\exported}[1]{{\color{lgray} \sf  [#1]}}


\newcommand{\gvarc}{\arc_{\bullet}(X,\lambda,\delta)}
\DeclareMathOperator{\injrad}{injrad}
\DeclareMathOperator{\Thick}{Thick}
\DeclareMathOperator{\Thin}{Thin}
\DeclareMathOperator{\Dil}{Dil}
\DeclareMathOperator{\sys}{sys}
\DeclareMathOperator{\Hor}{Hor}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\odd}{odd}
\DeclareMathOperator{\Mirz}{Mirz}

\newcommand{\wstarto}{\xrightharpoonup{*}}
\newcommand{\AIS}{\mathcal L}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bft}{\mathbf{T}}
\newcommand{\TRG}{\mathcal{TRG}}
\newcommand{\MRG}{\mathcal{MRG}}
\newcommand{\rg}{\mathsf{Y}}

\newcommand{\singodd}{\sing_{\odd}}

\newcommand{\bfl}{\boldsymbol\ell}
\newcommand{\bfh}{\mathbf{h}}

\newcommand{\Addresses}{{
  \bigskip
  \footnotesize
  \noindent Aaron Calderon, \textsc{Department of Mathematics, University of Chicago}\par\nopagebreak
  \textit{E-mail address}: \texttt{aaroncalderon@uchicago.edu}
  
  \noindent James Farre, \textsc{Max Planck Institute for Mathematics in the Sciences, Leipzig}\par\nopagebreak
  \textit{E-mail address}: \texttt{james.farre@mis.mpg.de}
  }}
